Energy-Efficient Resource Management in Microservices-based Fog and Edge Computing: State-of-the-Art and Future Directions

The exponential growth of Internet of Things (IoT) devices has intensified the demand for efficient and responsive services. To address this demand, fog and edge computing have emerged as distributed paradigms that bring computational resources closer to end users, reducing latency, bandwidth limitations, and energy consumption. However, these paradigms present challenges in resource management due to resource constraints, computational heterogeneity, dynamic workloads, and diverse Quality of Service (QoS) requirements. This paper presents a comprehensive survey of state-of-the-art resource management strategies in microservices-based fog and edge computing, focusing on energy-efficient solutions. We systematically review and classify more than 136 studies (2020-2024) into five key subdomains: service placement, resource provisioning, task scheduling and offloading, resource allocation, and instance selection. Our categorization is based on optimization techniques, targeted objectives, and the strengths and limitations of each approach. In addition, we examine existing surveys and identify unresolved challenges and gaps in the literature. By highlighting the lack of synergy among fundamental resource management components, we outline promising research directions leveraging AI-driven optimization, quantum computing, and serverless computing. This survey serves as a comprehensive reference for researchers and practitioners by providing a unified and energy-aware perspective on resource management in microservices-based fog and edge computing, paving the way for more integrated, efficient, and sustainable future solutions.

==> Files/Tables/T2Placement.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}

        \rowcolor[rgb]{0.753,0.753,0.753} 
\begin{sideways}Article\end{sideways} & 
\begin{sideways}Energy Consumption ~ ~  \end{sideways} & 
\begin{sideways}Energy Efficiency\end{sideways} & 
\begin{sideways}QoS (Response Time)\end{sideways} & 
\begin{sideways}Cost Minimization\end{sideways} & 
\begin{sideways}Latency\end{sideways} & 
\begin{sideways}Load Balancing\end{sideways} & 
\begin{sideways}Network Usage\end{sideways} & 
\begin{sideways}Service Time\end{sideways} & 
\begin{sideways}Reliability\end{sideways} & 
\begin{sideways}Fog Node Utilization\end{sideways} & 
\begin{sideways}Task Migration\end{sideways} & 
\begin{sideways}Throughput\end{sideways} & 
\begin{sideways}Service Delay\end{sideways}  & 
\begin{sideways}Fog/Edge/Hybrid \end{sideways} & 
\begin{sideways} Heuristic-Based Algorithms\end{sideways} & 
\begin{sideways}  Metaheuristic-Based Algorithms\end{sideways} & 
\begin{sideways}Optimization-Based Algorithms \end{sideways} & 
\begin{sideways}Machine Learning-Based Algorithms \end{sideways} & 
\begin{sideways}Graph-Based Algorithms \end{sideways} & 
\begin{sideways}Hybrid Algorithms \end{sideways} & 
\begin{sideways}Other \end{sideways} 
 
  \\ 
  \hline
    1.Kayal et al.~\cite{kayal2019autonomic} & \checkmark & \checkmark & ~ & \checkmark & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & Fog & ~ & \checkmark & \checkmark & ~ & ~ & ~ & ~ \\ \hline
        2.Hassan et al.~\cite{hassan2020priority} & \checkmark & \checkmark & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & Fog & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        3.Zeng et al.~\cite{zeng2020towards} & \checkmark & \checkmark & ~ & \checkmark & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & Fog & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        4.Goudarzi et al.~\cite{goudarzi2021distributed} & \checkmark & ~ & ~ & \checkmark & ~ & ~ & ~ & \checkmark & ~ & ~ & \checkmark & ~ & \checkmark & Hybrid & ~ & ~ & \checkmark & \checkmark & ~ & ~ & ~ \\ \hline
        5.Natesha et al.~\cite{natesha2021adopting} & \checkmark & \checkmark & ~ & \checkmark & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & Fog & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        6.Wang et al.~\cite{wang2021effective} & \checkmark & ~ & ~ & \checkmark & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & Edge & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        7.Ahvar et al.~\cite{ahvar2021deca} & \checkmark & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & Edge & ~ & ~ & ~ & ~ & ~ & \checkmark & \checkmark \\ \hline
        8.Thanh et al.~\cite{thanh2021energy} & \checkmark & \checkmark & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & Hybrid & \checkmark & ~ & \checkmark & ~ & ~ & ~ & ~ \\ \hline
        9.Tzenetopoulos et al.~\cite{tzenetopoulos2021fade} & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & Edge & \checkmark & ~ & \checkmark & ~ & ~ & ~ & ~ \\ \hline
        10.Cao et al.~\cite{cao2021large} & \checkmark & ~ & ~ & ~ & \checkmark & \checkmark & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & Edge & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        11.Santos et al.~\cite{santos2021reinforcement} & \checkmark & \checkmark & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & Fog & ~ & ~ & \checkmark & \checkmark & ~ & ~ & ~ \\ \hline
        12.Ghobaei-Arani et al.~\cite{ghobaei2022cost} & \checkmark & \checkmark & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & Fog & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        13.Mortazavi et al.~\cite{mortazavi2022discrete} & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & Fog & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        14.Zhao et al.~\cite{zhao2022qos} & \checkmark & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark & Fog & ~ & \checkmark & ~ & ~ & ~ & ~ & \checkmark \\ \hline
        15.Premsankar et al.~\cite{premsankar2022energy} & \checkmark & \checkmark & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & Edge & \checkmark & ~ & \checkmark & ~ & ~ & ~ & ~ \\ \hline
        16.Natesha et al.~\cite{natesha2022meta} & \checkmark & \checkmark & ~ & \checkmark & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & Fog & ~ & \checkmark & ~ & ~ & ~ & \checkmark & ~ \\ \hline
        17.Liu et al.~\cite{liu2022solving} & \checkmark & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ & \checkmark & Hybrid & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        18.Ray et al.~\cite{ray2023adaptive} & \checkmark & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark & Edge & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark \\ \hline
        19.e\{HU2023 et al.~\cite{HU2023} & \checkmark & \checkmark & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & Hybrid & ~ & \checkmark & ~ & ~ & ~ & \checkmark & ~ \\ \hline
        20.Singh et al.~\cite{singh2023integrated} & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & \checkmark & Fog & ~ & \checkmark & ~ & ~ & ~ & \checkmark & ~ \\ \hline
        21.Asghari et al.~\cite{asghari2023energy} & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark & ~ & Edge & ~ & \checkmark & ~ & ~ & ~ & \checkmark & ~ \\ \hline
        22.Rajagopal et al.~\cite{rajagopal2023fedsdm} & \checkmark & ~ & ~ & \checkmark & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & Hybrid & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ \\ \hline
        23.Zare et al.~\cite{zare2024imperialist} & \checkmark & \checkmark & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark & \checkmark & ~ & Fog & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        24.Srichandan et al.~\cite{srichandan2024secure} & \checkmark & \checkmark & ~ & \checkmark & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & Hybrid & ~ & \checkmark & ~ & \checkmark & ~ & ~ & ~ \\ \hline
        25.Dogani et al.~\cite{dogani2024two} & \checkmark & ~ & ~ & \checkmark & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & Fog & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        26.Kumar et al.~\cite{kumar2024auction} & \checkmark & ~ & ~ & ~ & ~ & \checkmark & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & Fog & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ \\ \hline
        27.Afachao et al.~\cite{afachao2024efficient} & \checkmark & ~ & ~ & ~ & ~ & \checkmark & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & Hybrid & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ \\ \hline
        28.Taleb et al.~\cite{taleb2024energy} & \checkmark & \checkmark & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & \checkmark & Hybrid & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        29.Sharma et al.~\cite{sharma2024intelligent} & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark & ~ & \checkmark & ~ & ~ & ~ & Fog & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ \\ \hline
        30.Ghasemi et al.~\cite{ghasemi2024mohho} & \checkmark & ~ & ~ & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ & \checkmark & \checkmark & ~ & Fog & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ \\ \hline
        31.Ghasemzadeh et al.~\cite{ghasemzadeh2025optimizing} & \checkmark & ~ & ~ & ~ & \checkmark & \checkmark & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & Edge & ~ & \checkmark & ~ & ~ & ~ & \checkmark & ~ \\ \hline
        32.Liang et al.~\cite{liang2024sustainable} & \checkmark & ~ & ~ & \checkmark & ~ & ~ & ~ & ~ & ~ & \checkmark & ~ & ~ & ~ & Edge & ~ & ~ & \checkmark & ~ & \checkmark & ~ & ~ \\ \hline
    \end{tabular}
\end{table}

==> Files/Tables/temp.tex <==
\begin{table}[!ht]
\caption{Temp Table} 
    \centering
    \begin{tabular}{|l|l|l|}
    \hline
        Placement. & Mathematical Based & ~\cite{ahvar2021deca},~\cite{qu2021service},~\cite{kumar2024auction},~\cite{arzo2024softwarized},~\cite{liang2024sustainable},~\cite{goudarzi2021distributed},~\cite{premsankar2022energy},~\cite{ray2023adaptive},~\cite{omer2021priority} \\ \hline
        Placement. & ML-Based & ~\cite{singh2023integrated},~\cite{srichandan2024secure},~\cite{rajagopal2023fedsdm},~\cite{afachao2024efficient},~\cite{sharma2024intelligent} \\ \hline
        Placement. & Heuristic-Based & ~\cite{ahvar2021deca},~\cite{qu2021service},~\cite{goudarzi2021distributed},~\cite{premsankar2022energy},~\cite{ray2023adaptive},~\cite{hassan2020priority},~\cite{zeng2020towards},~\cite{thanh2021energy},~\cite{tzenetopoulos2021fade},~\cite{song2023sd},~\cite{taleb2024energy},~\cite{fang2020iot},~\cite{ahmed2023ecq}
 \\ \hline
        Placement. & Metaheuristic-Based & ~\cite{singh2023integrated},~\cite{srichandan2024secure},~\cite{fang2020iot},~\cite{natesha2021adopting},~\cite{wang2021effective},~\cite{ghobaei2022cost},~\cite{mortazavi2022discrete},~\cite{zhao2022qos},~\cite{natesha2022meta},~\cite{liu2022solving},~\cite{HU2023},~\cite{asghari2023energy},~\cite{zare2024imperialist},~\cite{dogani2024two},~\cite{ghasemi2024mohho} \\ \hline
        Provisioning. & Mathematical Based & ~\cite{qu2021service},~\cite{canete2022proactive},~\cite{mays2022intent},~\cite{santos2021towards},~\cite{li2021cost},~\cite{das2022all} \\ \hline
        Provisioning. & ML-Based & ~\cite{hazra2021collaborative},~\cite{xiang2023dynamic},~\cite{faraji2022self},~\cite{mekki2023xai},~\cite{nandhakumar2024edgeaisim},~\cite{nizamis2024enact},~\cite{choupani2025joint}
 \\ \hline
        Provisioning. & Heuristic-Based & ~\cite{qu2021service},~\cite{li2021cost},~\cite{das2022all},~\cite{siasi2020delay},~\cite{adeppady2023energy},~\cite{choupani2025joint}
 \\ \hline
        Provisioning. & Metaheuristic-Based & ~\cite{xu2022dynamic},~\cite{rajagopal2023resource} \\ \hline
        Scheduling. & Mathematical Based & ~\cite{hazra2020joint},~\cite{zhao2021dynamic},~\cite{luo2021optimization},~\cite{samanta2020dyme},~\cite{mays2023federated},~\cite{yin2024joint},~\cite{raju2023delay},~\cite{zhao2024ets},~\cite{zou2024fine},~\cite{syrigos2023eelas} \\ \hline
        Scheduling. & ML-Based & ~\cite{raju2023delay},~\cite{zhao2024ets},~\cite{shruthi2022mayfly},~\cite{lakhan2022federated},~\cite{vijayalakshmi2023reinforcement},~\cite{murtaza2020qos},~\cite{tuli2021cosco},~\cite{seo2021slo},~\cite{sellami2022deep},~\cite{wang2023cloud},~\cite{filinis2024intent} \\ \hline
        Scheduling. & Heuristic-Based & ~\cite{hazra2020joint},~\cite{lakhan2022federated},~\cite{vijayalakshmi2023reinforcement},~\cite{zou2024fine},~\cite{syrigos2023eelas},~\cite{ijaz2021energy},~\cite{hosseini2022optimized},~\cite{azizi2022deadline},~\cite{aslanpour2022energy},~\cite{singh2022energy},~\cite{hosseini2023energy},~\cite{verma2024lease},~\cite{huang2023satedge},~\cite{ali2024edgebus},~\cite{shukla2024motors},~\cite{mahapatra2024energy} \\ \hline
        Scheduling. & Metaheuristic-Based & ~\cite{shruthi2022mayfly},~\cite{krishnan2024reliability},~\cite{abdel2020energy},~\cite{abdel2020energy},~\cite{buneman1997semistructured},~\cite{bali2023effective},~\cite{shukla2024motors},~\cite{mahapatra2024energy},~\cite{ijaz2025energy}~\cite{hoseiny2021pga},~\cite{dabiri2022optimizing},~\cite{karami2024bi},~\cite{salimi2024greedy}
 \\ \hline
        Allocation. & Mathematical Based & ~\cite{zhao2021energy},~\cite{chang2020dynamic},~\cite{zhang2020dynamic},~\cite{li2020energy},~\cite{alharbi2022energy},~\cite{mohajer2022heterogeneous},~\cite{zhou2022service},~\cite{bebortta2023optimal},~\cite{vahabi2023energy},~\cite{fe2023model},~\cite{sun2020energy},~\cite{qu2021service},~\cite{bellal2024gas},~\cite{xu2020energy},~\cite{fan2021cloud} \\ \hline
        Allocation. & ML-Based & ~\cite{tong2020adaptive},~\cite{zhu2021energy},~\cite{seid2021multi},~\cite{santos2021reinforcement},~\cite{santos2021resource},~\cite{mekala2022drl},~\cite{wang2023cloud},~\cite{lingayya2024dynamic} \\ \hline
        Allocation. & Heuristic-Based & ~\cite{sun2020energy},~\cite{qu2021service},~\cite{lingayya2024dynamic},~\cite{xu2020energy},~\cite{fan2021cloud},~\cite{yadav2020energy},~\cite{mahmud2021pi},~\cite{kumar2024auction},~\cite{yuan2020profit} \\ \hline
        Allocation. & Metaheuristic-Based & ~\cite{lingayya2024dynamic},~\cite{yuan2020profit},~\cite{li2021computation},~\cite{abbasi2021intelligent},~\cite{cao2021large},~\cite{apat2024hybrid},~\cite{liu2024multi},~\cite{ghasemzadeh2025optimizing} \\ \hline
        Replica Sel. & Mathematical Based & ~\cite{satar2022best},~\cite{sun2024minimizing},~\cite{wang2022service} \\ \hline
        Replica Sel. & ML-Based & ~\cite{hu2024joint},~\cite{ahmed2024neil},~\cite{liu2021virtual},~\cite{guo2023deep} \\ \hline
        Replica Sel. & Heuristic-Based & ~\cite{hu2024joint},~\cite{ahmed2024neil},~\cite{xie2020bandwidth},~\cite{fahs2020voila},~\cite{dias2021adaptive},~\cite{zhao2021temperature},~\cite{sethunath2022joint},~\cite{zhao2024winning},~\cite{jaradat2020multiple} \\ \hline
        Replica Sel. & Metaheuristic-Based & ~\cite{jaradat2020multiple},~\cite{zou2021towards},~\cite{wang2022service} \\ \hline
    \end{tabular}
\end{table}
